Non-oblivious Strategy Improvement

We study strategy improvement algorithms for mean-payoff and parity games. We describe a structural property of these games, and we show that these structures can affect the behaviour of strategy improvement. We show how awareness of these structures can be used to accelerate strategy improvement algorithms. We call our algorithms non-oblivious because they remember properties of the game that they have discovered in previous iterations. We show that non-oblivious strategy improvement algorithms perform well on examples that are known to be hard for oblivious strategy improvement. Hence, we argue that previous strategy improvement algorithms fail because they ignore the structural properties of the game that they are solving.

==> policy.tex <==
\section{Non-oblivious Switching Policies}
\label{policysection}

The purpose of this section is to define some non-oblivious switching policies.
In particular, we will show how to construct a non-oblivious version of an
oblivious switching policy. These policies will later be useful in
demonstrating how non-oblivious strategy improvement is not vulnerable to the
techniques used to prove lower bounds for oblivious strategy improvement. In
order to define reasonable switching policies we must first understand how our
choice of action affects the valuations of the vertices. The first part of this
section is dedicated to proving bounds for this.

Recall that the most common variant of all-switches, given in
Equation~\eqref{allswitches} breaks ties by choosing the successor with the
highest valuation. Although this may seem arbitrary, the justification for this
choice is the following well-known lower bound: after switching an edge $(v, u)$
in a strategy $\sigma$ the valuation of $v$ will increase by at least the
difference between the valuation of $\sigma(v)$ and $u$. Formally we define the
increase of a profitable edge $(v, u)$ in a strategy $\sigma$ as
$\increase^{\sigma}(v, u) = \val^{\sigma}(u) - \val^{\sigma}(\sigma(v))$. We can
now show that the valuation of some vertex will increase by at least this amount
when switching the profitable edge.

\begin{proposition}
\label{lowerbound}
Let $(v, u)$ be a profitable edge in a strategy $\sigma$. After switching the
edge we have $\val^{\sigma[v \mapsto u]}(v) - \val^{\sigma}(v) \ge \increase^{\sigma}(v, u)$. 
\end{proposition}

Proposition~\ref{lowerbound} gives a lower bound on the increase in valuations
that switching a profitable edge causes. In general the actual increase in
valuation can far exceed the increase implied by this lower bound. We show that
the increase in valuation depends on the type of edge that is being switched.
Our first task is to show that for profitable cross edges the lower bound given
in Proposition~\ref{lowerbound} is actually correct. 

\begin{proposition}
\label{upperboundce}
Let~$(v, u)$ be a profitable cross edge in the strategy~$\sigma$. For every
vertex $w$ we have $\val^{\sigma[v \mapsto u]}(w) - \val^{\sigma}(w) \le
\increase^{\sigma}(v, u)$
\end{proposition}

While the lower bound given by Proposition~\ref{lowerbound} is tight for cross
edges, it significantly under estimates the increase in valuation caused by a
back edge. We will use our results from Section~\ref{pbe} to provide an improved
lower bound for this increase. Recall that Proposition~\ref{chooseescape}
implies that Min must choose an escape from the critical set of the back edge in
the best response of the next iteration. For each escape $(x, y)$ from the
critical set of a back edge we define the increase of that escape to be the
difference between the valuation of $x$ and the valuation of $y$ plus the weight
of $x$.  We then define the escape increase of a profitable back edge $(v, u)$
to be the minimum over the increases of the escapes from the critical set of
that back edge. Formally, we have $\ei(v, u) = \min\{(\val^{\sigma}(y) +
\weight(x)) - \val^{\sigma}(x) \; : \; (x, y) \in \escapes(\critical^{\sigma}(v,
u))\}$. We now define a better lower bound for the increase of a profitable edge
$(v, u)$ which incorporates the escape increase of a profitable back edge. We
define $\newincrease^{\sigma}(v, u) = \max(\increase^{\sigma}(v, u), \ei(v, u))$
if $u \in \subtree^{\sigma}(v)$ and $\increase^{\sigma}(v, u)$ otherwise.

\begin{algorithm}
\begin{algorithmic}
\STATE $(v, u) := \argmax_{(x, y)} \newincrease^{\sigma}(x, y)$
\STATE $(W, \chi) := \argmax_{(X, \mu) \in S} \snareincrease^{\sigma}(X, \mu)$
\IF{$\newincrease^{\sigma}(v, u) > \snareincrease(W, \chi)$}
\STATE $P := \{ (v, u) \; : \; (v, u) \text{ is profitable in } \sigma \}$
\STATE $\sigma := \sigma[\alpha(P)]$
\ELSE
\STATE $\sigma := \fixsnare(\sigma, (W, \chi))$
\ENDIF
\STATE \textbf{return} $\sigma$
\end{algorithmic}
\caption{$(\nonobv(\alpha))(\sigma, S)$}
\label{nonobv}
\end{algorithm}

\begin{proposition}
\label{lowerbe}
Let $(v, u)$ be a profitable edge in the strategy $\sigma$.
There is a vertex $w$ such that $\val^{\sigma[v \mapsto u]}(w) -
\val^{\sigma}(w) \ge \newincrease^{\sigma}(v, u)$.
\end{proposition}

Finally, we use similar techniques to give a snare increase operator, which
gives a lower bound for the increase in valuation that is obtained running the
$\fixsnare$ procedure. Let $(W, \chi)$ be a snare and suppose that the current
strategy is $\sigma$. We define $\snareincrease^\sigma(W, \chi) =
\min\{(\val^{\sigma}(y) + \weight(x)) - \val^{\sigma}(x) \; : \; (x, y) \in
\escapes(W)\}$.

\begin{proposition}
\label{lowersnare}
Let~$\sigma$ be a strategy that is not consistent with a snare~$(W, \chi)$, and
let~$\sigma'$ be the result of $\fixsnare(\sigma, (W, \chi))$. There is some
vertex~$w$ such that $\val^{\sigma'}(w) - \val^{\sigma}(w) \ge \snareincrease(W,
\chi)$.
\end{proposition}

We can now define the switching policies that will be used in
Section~\ref{friedmann}. We begin by using our new bounds for the increase of
switching an edge to provide an improved, although still oblivious, version of
the all-switches policy. We define $\newall(F) = \{ (v, u) \; : \; $ There is no
edge $(v, w) \in F$ with $\newincrease^{\sigma}(v, u) < \newincrease^{\sigma}(v,
w)\}$. While this policy is still oblivious, we will show in the next section
that being aware of the effect of switching a back edge gives this policy an
advantage over the traditional all-switches policy in certain situations.

%\begin{algorithm}
%\begin{algorithmic}
%\STATE $(v, u) := \argmax_{(x, y)} \increase^{\sigma}(x, y)$
%\STATE $(W, \chi) := \argmax_{(X, \mu) \in S} \snareincrease^{\sigma}(X, \mu)$
%\IF{$\increase^{\sigma}(v, u) > \snareincrease(W, \chi)$}
%\STATE $\sigma := \sigma[v \mapsto u]$
%\ELSE
%\STATE $\sigma := \fixsnare(\sigma, (W, \chi))$
%\ENDIF
%\STATE \textbf{return} $\sigma$
%\end{algorithmic}
%\caption{$\nonobsingle(\sigma, S)$}
%\label{nonobsingle}
%\end{algorithm}

%We now turn our attention to non-oblivious strategy improvement switching
%policies. The simplest type of policy is one that, in each iteration, either
%switches a profitable edge or runs $\fixsnare$ on some snare. We will give one
%such policy that picks, from the snares and profitable edges, the action that
%provides the largest increase in valuation as given by our bounds. This
%switching policy is shown as Algorithm~\ref{nonobsingle}.

We now give one method of deriving a non-oblivious switching policy from an
oblivious one. Given an oblivious switching policy $\alpha$ we define
$\nonobv(\alpha)$ to be the switching policy shown as Algorithm~\ref{nonobv}.
The idea here is to compare the increases that would be gained by switching
profitable edges and by fixing snares. If making the current strategy consistent
with a snare yields a larger increase than switching an edge then the policy
will call $\fixsnare$ for that snare. Otherwise, the policy switches the edges
that would be switched by $\alpha$. This allows us to define a non-oblivious
version of all switches as $\nonobv(\newall)$, which will be useful in the next
section.

%This follows the same idea as the single switch
%policy. The difference is that, when switching an edge gives a better increase
%in the valuation than fixing a snare, the policy runs $\alpha$. 

